CLIPtortionist: Zero-shot Text-driven Deformation for Manufactured 3D Shapes

We propose a zero-shot text-driven 3D shape deformation system that deforms an input 3D mesh of a manufactured object to fit an input text description. To do this, our system optimizes the parameters of a deformation model to maximize an objective function based on the widely used pre-trained vision language model CLIP. We find that CLIP-based objective functions exhibit many spurious local optima; to circumvent them, we parameterize deformations using a novel deformation model called BoxDefGraph which our system automatically computes from an input mesh, the BoxDefGraph is designed to capture the object aligned rectangular/circular geometry features of most manufactured objects. We then use the CMA-ES global optimization algorithm to maximize our objective, which we find to work better than popular gradient-based optimizers. We demonstrate that our approach produces appealing results and outperforms several baselines.

==> 02-related.tex <==
\section{Related Work}
%
Our work is related to prior work on deformation-based shape editing, shape approximation, and text-driven shape optimization.
Although outside of our scope, we also briefly discuss recent progress on text-driven shape generation.

\subsection{Deformation-based shape editing}
%
The seminal work in this area formulated deformation-based shape editing as constrained optimization: optimizing shapes to respect user-provided constraints (such as positions of mesh vertices) while minimizing some measure of distortion to the mesh~\cite{ARAP_modeling:2007,ARAPIgarashi,intuitive_edit,MovingFrameManipulation,PoissonGradientMeshEditing,HarmonicGuidance,DualLaplacian,BoundedBiharmonicWeights}
Recent advances in deep neural networks have led to learning-based methods for deformation-based shape editing.
One popular fomluation is learning to predict deformations which deform a given source shape toward a given target shape~\cite{Yifan:NeuralCage:2020,LearningFreeformDef,groueix19cycleconsistentdeformation,wang20193dn}
These methods requires a dataset of target shapes as supervision for training the deformation model, whereas as our method assumes only a single source shape as input.
DeepMetaHandles~\cite{liu2021deepmetahandles} and KeypointDeformer~\cite{keypointdeformer} automatically learn semantic shape editing handles from a dataset of shapes of the same category; again, these methods both require a large collection of shapes as input.
In addition, the deformation handles they produce will not necessarily align with or support a particular semantic edit that a user wants to perform.
Our system produces a semantic deformer for a specific text prompt, given only a single mesh as input.
 
\subsection{Shape approximation}
%
Many methods have been proposed to approximate 3D shapes.
Several approaches approximate 3D shapes as collections of cuboids~\cite{abstractionTulsiani17,sun2019abstraction,yang2021unsupervised}.
One can also obtain more geometric flexibility by approximating 3D shapes using geometric primitives other than cuboids.
Prior work has investigated automatic/unsupervised shape approximation using superquadrics~\cite{Paschalidou2019CVPR}, convex polyhedra~\cite{deng2020cvxnet}, and deformed sphere meshes~\cite{Paschalidou2021CVPR}.
Our deformation model, BoxDefGraph, can be seen as a type of shape approximation/proxy.
It is based on prior work by Xian et al. which automatically generates part-level AABBs to approximate a 3D shape~\cite{autoOBB}.
We modify their method to produce AABBs that are well-suited for optimizing deformations with respect to a CLIP objective, including novel algorithms for imposing constraints between AABB parameters as a constraint graph and also turning the resulting constraint graph into a tree that can be solved mostly in closed form.

\subsection{Text-Driven Shape Generation and Editing}
%
The Semantic Shape Editing system~\cite{semantic_shape} produces compelling deformations of a shape to increase or decrease the degree to which that shape satisfies some semantic attribute (e.g. a ``sporty'' car). However, it requires carefully designed part-level shape deformers, and its optimization objective is derived from a large-scale human perceptual study which gathered pairwise judgments of 3D shapes. Follow-on work replaced the part-level deformers with a deformation field predicted by a neural network~\cite{yumer2016learning}.
With the recent emergence of large-scale pretrained vision-language models such as CLIP~\cite{clip2021}, it is possible to approach the text-based shape editing problem without collecting such large-scale training data. The Text2Mesh system modifies a mesh's vertex positions and colors to maximize a CLIP similarity score~\cite{text2mesh}. However, it is limited to producing small-scale displacements of mesh vertices to change the shape's perceived ``style'' and cannot produce large coherent changes to overall geometry. The TextDeformer system modifies a mesh's face Jacobians to maximize a CLIP similarity score ~\cite{Gao_2023_SIGGRAPH}. However, it changes the surface details and sometimes structure of the mesh and destroys the mesh's identity. Our system produces such large shape changes while preserving the surface details and also leveraging CLIP to eliminate the need for supervised training data.

There is also a large and growing body of work on text-based shape \emph{generation}, including methods based on supervised learning~\cite{chen2018text2shape,autosdf2022,fu2022shapecrafter} as well as those which use CLIP to operate in a zero-shot fashion~\cite{sanghi2021clip,jain2021dreamfields,poole2022dreamfusion}.
These methods aim to synthesize new shapes from a text prompt, whereas ours deforms an existing shape.


==> 08-conclusion.tex <==
   
